Renewal theorems for a class of processes with dependent interarrival times and applications in geometry

Renewal theorems are developed for point processes with interarrival times $W_n=\xi(X_{n+1}X_n\cdots)$, where $(X_n)_{n\in\mathbb Z}$ is a stochastic process with finite state space $\Sigma$ and $\xi\colon\Sigma_A\to\mathbb R$ is a H\"older continuous function on a subset $\Sigma_A\subset\Sigma^{\mathbb N}$. The theorems developed here unify and generalise the key renewal theorem for discrete measures and Lalley's renewal theorem for counting measures in symbolic dynamics. Moreover, they capture aspects of Markov renewal theory. The new renewal theorems allow for direct applications to problems in fractal and hyperbolic geometry; for instance, results on the Minkowski measurability of self-conformal sets are deduced. Indeed, these geometric problems motivated the development of the renewal theorems.

==> applications.tex <==
In this section we briefly describe one application of the Renewal \cref{thm:RT1}, namely the existence of the Minkowski content of self-conformal sets. It is this application which lead to developing \cref{thm:RT1}. Here, we will not give a full account of the problem and the precise assumptions, but merely focus on the general ideas behind its solution. For the details and the precise setting we refer the reader to \cite{Diss} or a forthcoming article by the author.

Let $B\subset\mathbb R^d$ denote a bounded subset of the $d$-dimensional Euclidean space $(\mathbb R^d,\|\cdot\|_2)$. 
The \emph{Minkowski content} of $B$ describes the asymptotic behaviour of the ($\ee^{-t}$)-parallel volume $\lambda_d(B_{\ee^{-t}})$ of $B$ as $t\to\infty$. Here $B_{\ee^{-t}}\defeq\{x\in\mathbb R^d\mid\inf_{b\in B}\|b-x\|_2\leq \ee^{-t}\}$ and $\lambda_d$ denotes the $d$-dimensional Lebesgue measure. More precisely, the Minkowski content $\mathcal{M}(B)$ of $B$ is defined by
\[
  \mathcal{M}(B)\defeq\lim_{t\to\infty}\ee^{t(d-D)}\lambda_d(B_{\ee^{-t}}),
\]
whenever this limit exists, where $D\defeq d+\lim_{t\to\infty}t^{-1}\log\lambda_d(B_{\ee^{-t}})$ denotes the Minkowski dimension of $B$. Notice, the definition of the Minkowski content implicitly assumes that the Minkowski dimension exists. (The Minkowski dimension coincides with the box-counting dimension, see \cite[Proposition 3{.}2]{Falconer}.) If $B$ is a set with $\lambda_d(B)>0$ then the definitions imply that $D=d$ and that $\mathcal M(B)=\lambda_d(B)$. If $D<d$ then $\lambda_d(B)=0$ and the Minkowski content, when it exists, can be viewed as the $D$-dimensional volume of $B$ and hence as a substitute of the notion of volume. Besides this geometric relevance, the Minkowski content plays a major role in the Weyl-Berry conjecture, which is concerned with spectral asymptotics of Laplace operators on domains with irregular boundaries. These are two of the reasons why the Minkowski content has attracted much attention in recent years (see for instance \cite{survey} for a more in depth introduction to the Minkowski content).

Self-conformal sets are defined as follows. Take $X\subset\mathbb R^d$ to be a compact non-empty set satisfying $X=\overline{\inte X}$. Define $\Phi\defeq\{\phi_1,\ldots,\phi_M\colon X\to X\}$ to be an iterated function system (IFS) consisting of contractive conformal $\mathcal C^{1+\alpha}$-diffeomorphisms $\phi_i$ with $M\geq 2$. (A special case occurs if $\phi_1,\ldots,\phi_M$ are contractive similtudes, that is if $\|\phi_i(x)-\phi_i(y)\|_2=c_i\|x-y\|_2$ for all $x,y\in X$ and $i\in\{1,\ldots,M\}$ with $c_i\in(0,1)$.)
We let $F$ denote the unique compact non-empty invariant set of the IFS $\Phi$, that is the unique compact non-empty set $F$ satisfying $F=\bigcup_{i=1}^M \phi_i F$. This exists due to \cite{Hutchinson} and is called the \emph{self-conformal set} associated with $\Phi$. If $\phi_1,\ldots,\phi_M$ are similtudes, then $F$ is called \emph{self-similar}.
Self-similar and self-conformal sets provide prominent examples of fractal sets, see \cref{ex:pictures} and \cref{fig:fractals}.

\begin{figure}
   \begin{subfigure}[c]{0.3\textwidth}
   \includegraphics[width=\textwidth]{Sierpgasket}
   \subcaption{}
   \label{fig:Sierp_gasket}
   \end{subfigure}
   \quad
   \begin{subfigure}{0.3\textwidth}
   \includegraphics[width=\textwidth]{bat}
   \subcaption{}
   \label{fig:bat}
   \end{subfigure}
   \quad
   \begin{subfigure}{0.3\textwidth}
   \includegraphics[width=\textwidth]{t01}
   \subcaption{}
   \label{fig:moeb1}
   \end{subfigure}
   \caption{The self-conformal sets which are described in \cref{ex:pictures}: 
   \subref{fig:Sierp_gasket} The Sierpinski gasket -- an example of a self-similar set.
   \subref{fig:bat} and \subref{fig:moeb1} Conformal images of the Sierpinski gasket -- examples of self-conformal sets which are not self-similar. The figures are created with matlab.}
   \label{fig:fractals}
\end{figure}

Next, we describe the general ideas of how  \cref{thm:RT1} can be used to obtain the asymptotic behaviour of $\lambda_d(F_{\ee^{-t}})$ as $t\to\infty$, resulting in statements on the existence of the Minkowski content, for a self-conformal set $F$. For this, we now give an overview of some main assumptions, which are necessary to understand the link between the Minkowski content and the renewal theorem. For more details, the reader is referred to \cite{Diss,survey,Steffen_gamma}.
Assume that $\Phi$ satisfies the open set condition (OSC), that is there exists a \emph{feasible open set} $O\subset X$, which is non-empty, open and satisfies $\phi_i O\subset O$ as well as $\phi_i O\cap \phi_j O=\emptyset$ for $i\neq j\in\{1,\ldots,M\}\eqdef\Sigma$. Set $\Gamma\defeq O\setminus\bigcup_{i=1}^M \phi_i O$, $\Phi\Gamma\defeq\bigcup_{i=1}^M\phi_i\Gamma$ and note that
\begin{align}\label{eq:OUplus}
  O=\bigcup_{n=0}^{\infty}\bigcup_{u\in\Sigma^n}\phi_u\Gamma\cup\bigcap_{n=0}^{\infty}\Phi^n O,
\end{align}
where the unions are disjoint. 
For the sets from \cref{fig:fractals} examples of sets $O$, with associated sets $\Phi O$ and $\Gamma$ are depicted in \cref{fig:opengamma}.
We have $\Phi\left(\overline{\bigcap_{n=0}^{\infty}\Phi^n O}\right)=\overline{\bigcap_{n=0}^{\infty}\Phi^n O}$. Thus, $\overline{\bigcap_{n=0}^{\infty}\Phi^n O}$ is compact and invariant, whence it is either empty or coincides with $F$ by uniqueness of the self-conformal set. Therefore, $\lambda_d\left(\bigcap_{n=0}^{\infty}\Phi^n O\right)\leq \lambda_d(F)$.
Let $D$ denote the Minkowski dimension of $F$ and assume that $D<d$. Then $ \lambda_d(F)=0$ by definition of $D$, whence
\begin{equation}\label{eq:restzero}
	\lambda_d\left(\bigcap_{n=0}^{\infty}\Phi^n O\right)=0.
\end{equation}
Suppose that $O$ can be chosen so that $\lambda_d(F_{\ee^{-t}}\cap\Gamma)\in\mathfrak{o}(\ee^{t(D-d)})$ with the Landau symbol $\mathfrak o$. 
\renewcommand\thesubfigure{}
\begin{figure}
   \begin{subfigure}{0.25\textwidth}
        \includegraphics[width=\textwidth]{Sierpgasket}
        \includegraphics[width=\textwidth]{bat}
        \includegraphics[width=\textwidth]{t01}
   \caption{$F$}
   \end{subfigure}
   \hspace{-0.25cm}
   \begin{subfigure}{0.25\textwidth}
        \includegraphics[width=\textwidth]{Sierpinskigasket_openset}
        \includegraphics[width=\textwidth]{bat_open}
        \includegraphics[width=\textwidth]{t01_open}
   \caption{$O$}
   \end{subfigure}
   \hspace{-0.25cm}
   \begin{subfigure}{0.25\textwidth}
      \includegraphics[width=\textwidth]{Sierpinskigasket_fopen}
      \includegraphics[width=\textwidth]{bat_fopen}
      \includegraphics[width=\textwidth]{t01_fopen}
   \caption{$\Phi O$}
   \end{subfigure}
   \hspace{-0.25cm}
   \begin{subfigure}{0.25\textwidth} 
      \includegraphics[width=\textwidth]{Sierpinskigasket_gamma}
      \includegraphics[width=\textwidth]{bat_gamma}
      \includegraphics[width=\textwidth]{t01_gamma}
   \caption{$\Gamma$}
   \end{subfigure}
   \caption{The self-conformal sets $F$ from \cref{ex:pictures} (see \cref{fig:fractals}), together with examples of associated feasible open sets $O$ and the respective sets $\Phi O$ and $\Gamma$.  The figures are created with matlab.}
    \label{fig:opengamma}
\end{figure}
For $\om=\om_1\cdots\om_n\in\Sigma^n$ write $\phi_{\om}\defeq\phi_{\om_1}\circ\cdots\circ\phi_{\om_n}$. Then by \eqref{eq:OUplus} and \eqref{eq:restzero} we have that
\begin{align*}
  \lambda_d(F_{\ee^{-t}}\cap O)
  &= \sum_{n=0}^{\infty}\sum_{u\in\Sigma^n}\lambda_d(F_{\ee^{-t}}\cap\phi_u\Gamma)\\
  &=\sum_{\om\in\Sigma^m}\sum_{n=0}^{\infty}\sum_{u\in\Sigma^n}\lambda_d(F_{\ee^{-t}}\cap\phi_u\phi_{\om}\Gamma)+\mathfrak{o}(\ee^{t(D-d)})
\end{align*}
for any $m\in\mathbb N$. By \cite{Steffen_gamma} we can always find a feasible open set $O$ so that $\lambda_d(F_{\ee^{-t}}\cap\phi_u\phi_{\om}\Gamma)=\lambda_d((\phi_uF)_{\ee^{-t}}\cap\phi_u\phi_{\om}\Gamma)$ and henceforth we suppose that $O$ satisfies this condition. In our examples from \cref{fig:fractals}, the open sets $O$, which are depicted in \cref{fig:opengamma}, satisfy the above conditions (see \cref{ex:pictures}). If $m$ is large, then the set $\phi_{\om}\Gamma$ is small, since each $\phi_i$ is strictly contracting. As conformal maps locally behave like similarities and $\lambda_d$ is homogeneous of degree $d$, we can approximate $\lambda_d((\phi_uF)_{\ee^{-t}}\cap\phi_u\phi_{\om}\Gamma)$ by 
\begin{equation}\label{eq:approxMink}
\lvert\phi_u'(\pi\sigma\om x)\rvert^d\lambda_d(F_{\ee^{-t}/\lvert\phi_u'(\pi\sigma\om x)\rvert}\cap\phi_{\om}\Gamma)
\end{equation}
 with an arbitrary $x\in\Sigma^{\mathbb N}$, where $\pi\colon\Sigma^{\mathbb N}\to F$ is the \emph{code map} defined by $\{\pi(\om)\}\defeq\bigcap_{n=0}^{\infty}\phi_{\om\vert_n}(X)$ and $\sigma$ is the shift-map as before. 
In order to bring \eqref{eq:approxMink} into a form to apply the renewal theorem we define $\codefun\colon\Sigma^{\mathbb N}\to\mathbb R$ by
\[
\codefun(\om)\defeq-\log\lvert\phi'_{\om_1}(\pi\sigma\om)\rvert.
\]
The function $\codefun$ is called the \emph{geometric potential function} associated with the IFS $\Phi$. It carries important geometric information of $\Phi$ and $F$.
Using the definition of $\codefun$ we see that $\exp(-S_n\codefun(u\om x))=\lvert\phi_u'(\pi\sigma\om x)\rvert$. Thus, $\lambda_d(F_{\ee^{-t}}\cap O)$ can be approximated by 
\[
\sum_{\om\in\Sigma^m}\sum_{n=0}^{\infty}\sum_{u\in\Sigma^n}\ee^{-dS_n\codefun(u\om x)}
\lambda_d(F_{\ee^{-t+S_n\codefun(u\om x)}}\cap\phi_{\om}\Gamma)+\mathfrak{o}(\ee^{t(D-d)}).
\]
Setting $f_y(t)\defeq\lambda_d(F_{\ee^{-t}}\cap\phi_{\om}\Gamma)$ for $y\in\Sigma^{\mathbb N}$, $\codefunc$ to be the constant one-function on $\Sigma^{\mathbb N}$, $\eta\defeq-d\codefun$ and assuming that Conditions \crefrange{it:Lebesgueintegrable}{it:regular} are satisfied, we can apply \cref{thm:RT1} and, for the case that $\codefun$ is non-lattice, obtain
\begin{align*}
  &\sum_{n=0}^{\infty}\sum_{u\in\Sigma^n}\ee^{-dS_n\codefun(u\om x)}
\lambda_d(F_{\ee^{-t+S_n\codefun(u\om x)}}\cap\phi_{\om}\Gamma)\\
  &\quad=N(t,\om x)\\
  &\quad\sim \ee^{t\mdim}\frac{\eigenf_{-(d+\mdim)\codefun}(\om x)}{\int\codefun\textup{d}\mu_{-(d+\mdim)\codefun}}\int_{-\infty}^{\infty}\ee^{-T\mdim}\lambda_d(F_{\ee^{-T}}\cap\phi_{\om}\Gamma)\textup{d}T,
\end{align*}
where $\mdim>0$ is the unique value for which $P(-(d+\mdim)\codefun)=0$. It is proven in \cite{Bedford} that the Minkowski dimension $D$ of $F$ is the unique solution to $P(-D\codefun)=0$ thus, $d+\mdim=D$. Using approximation arguments (based on bounded distortion properties of $\Phi$) we all in all obtain, in the non-lattice situation, that
\begin{align*}
  \lambda_d(F_{\ee^{-t}}\cap O)
  \sim\ee^{t(D-d)}\lim_{m\to\infty}\sum_{\om\in\Sigma^m}\frac{\eigenf_{-D\codefun}(\om x)}{\int\codefun\textup{d}\mu_{-D\codefun}}\int_{-\infty}^{\infty}\ee^{-T(D-d)}\lambda_d(F_{\ee^{-T}}\cap\phi_{\om}\Gamma)\textup{d}T
\end{align*}
(see \cite[Theorem 2{.}29]{Diss}). This shows that $\codefun$ being non-lattice implies existence of the Minkowski content which can be determined explicitly.
The lattice and the average cases can be treated similarly.

In the special case that $F$ is self-similar, the approximation arguments are not needed and $m$ can be assumed to be zero. Further, the eigenfunction $\eigenf_{-D\codefun}$ is the constant one-function on $\Sigma_A$, $\codefun$ is constant on cylinder sets of length one, taking the values $-\log(r_i)$ with $r_i\defeq\|\phi'_i\|_{\infty}$ and $\mu_{-D\codefun}([i])=r_i^D$. Therefore, for self-similar sets $F$ we obtain
\begin{align*}
  \lambda_d(F_{\ee^{-t}}\cap O)
  \sim\ee^{t(D-d)}\frac{1}{\sum_{i=1}^M-\log(r_i)r_i^D}\int_{-\infty}^{\infty}\ee^{-T(D-d)}\lambda_d(F_{\ee^{-T}}\cap\Gamma)\textup{d}T
\end{align*}
if $\codefun$ is non-lattice (see \cite[Theorem 2{.}37]{Diss}).
If $\codefun$ is lattice then the respective formula is more involved but we can easily deduce from \cref{thm:RT1} that
\begin{align}\label{eq:latticefractal}
\begin{aligned}
 &\lim_{t\to\infty}t^{-1}\int_0^t \ee^{-T(D-d)}\lambda_d(F_{\ee^{-t}}\cap O)\textup{d}T\\
 &\quad= \frac{1}{\sum_{i=1}^M-\log(r_i)r_i^D}\int_{-\infty}^{\infty}\ee^{-T(D-d)}\lambda_d(F_{\ee^{-T}}\cap\Gamma)\textup{d}T.
 \end{aligned}
\end{align}

\begin{example}[Examples of self-conformal sets]\label{ex:pictures}
	The self-conformal sets which are described here are depicted in \cref{fig:fractals,fig:opengamma}. In all the examples, $d=2$. We will discuss the Minkowski content for the first set \subref{fig:Sierp_gasket} and restrict ourselves to the definitions and verification of the main conditions for \subref{fig:bat} and \subref{fig:moeb1}.
	\begin{enumerate}[label=(\Alph*)]
		\item The Sierpinski gasket $F$, depicted in \cref{fig:fractals}\subref{fig:Sierp_gasket}, is the unique compact invariant set of the IFS $\Phi\defeq\{\phi_1,\phi_2,\phi_3\colon\mathbb R^2\to\mathbb R^2\}$ given by $\phi_1(x)=x/2$, $\phi_2(x)=x/2+(1/2,0)$ and $\phi_3(x)=x/2+(1/4,\sqrt{3}/4)$. Since $\phi_1$, $\phi_2$ and $\phi_3$ are similtudes it is a self-similar set. It is well-known that the Minkowski dimension of the Sierpinski gasket is $D=\log(3)/\log(2)$. The set $\Gamma$ is the equilateral triangle with vertices $(1/2,0)$, $(1/4,\sqrt{3}/4)$, $(3/4,\sqrt{3}/4)$, and 
		\[
		\lambda_2(F_{\ee^{-t}}\cap\Gamma)=
		\begin{cases}
			\tfrac{3}{2}\ee^{-t}-3\sqrt{3}\ee^{-2t}& :t>-\log(\sqrt{3}/12)\\
			\tfrac{\sqrt{3}}{16}&  :t\leq-\log(\sqrt{3}/12).
		\end{cases}
		\]
		Thus, $\lambda_2(F_{\ee^{-t}}\cap\Gamma)\in\mathfrak{o}(\ee^{t(D-2)})$.
		We have $r_i\defeq\|\phi'_i\|_{\infty}=1/2$ for $i\in\{1,2,3\}$. Hence, the system is lattice and \eqref{eq:latticefractal} yields that 
		\begin{align*}
		&\lim_{t\to\infty} t^{-1}\int_0^t \ee^{-T(D-2)}\lambda_2(F_{\ee^{-T}}\cap O)\textup{d}T\\
		&\quad= \frac{\sqrt{3}^{-(D+1)}}{\log(2)}\left[\frac{1}{2-D}+\frac{2}{D-1}-\frac{1}{D}\right]
		\approx 1{.}8126.
		\end{align*}
		\item The set $F$ depicted in \cref{fig:fractals}\subref{fig:bat} is the image of the Sierpinski gasket under the complex M\"obius transform $g_1\colon\mathbb{C}\to\mathbb C$, $z\mapsto-\im z/(\sqrt{3}z-\sqrt{3}-\im)$. An associated IFS is $\{g_1\circ\phi_i\circ g_1^{-1}\mid i\in\{1,2,3\}\}$ with $\phi_1,\phi_2,\phi_3$ being the similtudes which generate the Sierpinski gasket.  The maps $g_1\circ\phi_i\circ g_1^{-1}$ are contractive conformal $\mathcal{C}^{1+\alpha}$-diffeomorphisms, but not similtudes. Moreover, it can be shown that there does not exist an IFS consisting of similtudes which has $F$ as invariant set. Hence, $F$ is self-conformal but not self-similar. It is known that the Minkowski dimension is stable under bi-Lipschitz maps (see \cite[Theorem 9.3]{Falconer}). Thus, $D=\log(3)/\log(2)$. Since $\partial \Gamma$ is one-dimensional we have that $\lambda_2(F_{\ee^{-t}}\cap\Gamma)\in\mathfrak{O}(\ee^{-t})$ with the big Landau symbol $\mathfrak{O}$, whence $\lambda_2(F_{\ee^{-t}}\cap\Gamma)\in\mathfrak{o}(\ee^{t(D-d)})$.
		\item In \cref{fig:fractals}\subref{fig:moeb1} the image of the Sierpinski gasket under the complex M\"obius transform $g_2\colon\mathbb C\to\mathbb C$, $z\mapsto(1-\sqrt{3}\im)z/((12+10\sqrt{3}\im)z-11-11\sqrt{3}\im)$ is depicted.
		Analogous to \subref{fig:bat} an associated IFS is given by $\{g_2\circ\phi_i\circ g_2^{-1}\mid i\in\{1,2,3\}\}$ and $\lambda_2(F_{\ee^{-t}}\cap\Gamma)\in\mathfrak{O}(\ee^{-t})$.
	\end{enumerate}
\end{example}
